Multiresolution Mapping and Informative Path Planning for UAV-based Terrain Monitoring

Unmanned aerial vehicles (UAVs) can offer timely and cost-effective delivery of high-quality sensing data. How- ever, deciding when and where to take measurements in complex environments remains an open challenge. To address this issue, we introduce a new multiresolution mapping approach for informative path planning in terrain monitoring using UAVs. Our strategy exploits the spatial correlation encoded in a Gaussian Process model as a prior for Bayesian data fusion with probabilistic sensors. This allows us to incorporate altitude-dependent sensor models for aerial imaging and perform constant-time measurement updates. The resulting maps are used to plan information-rich trajectories in continuous 3-D space through a combination of grid search and evolutionary optimization. We evaluate our framework on the application of agricultural biomass monitoring. Extensive simulations show that our planner performs better than existing methods, with mean error reductions of up to 45% compared to traditional "lawnmower" coverage. We demonstrate proof of concept using a multirotor to map color in different environments.

==> Makefile <==
## Makefile to compile .tex files.
#
# Author: Gregory Hitz
#

## targets and dependencies
# by default all .tex will be converted into .pdf:
#targets=$(subst .tex,.pdf,$(wildcard *.tex))
targets=2017-iros-popovic.pdf

# definition of dependency directories
images_dir = images
ref_dir = references


# compilation feature switches. Should be 0 (off) or 1 (on). If the variables
# are set as environmnet variables they are read from there. otherwise the
# default values are assigned (after the minus sign)
# use_gs:				use ghostscript to postprocess the compiled pdf
#						(default = 1)
# fail_on_missing_refs: fail if pdflatex reports missing references
#						(default = 0)
# These settings can also be applied as arguments to the make call:
#		(e.g.: $ make use_gs=1)
# NOTE:	for this to work the env variables need to be exported
#		(e.g.: export USE_GS=1;)
use_gs = $(shell echo $${USE_GS:-1})
fail_on_missing_refs =  $(shell echo $${FAIL_ON_MISSING_REFS:-0})

deps= \
	  $(wildcard *.inc) \
	  $(wildcard $(images_dir)/*.pdf) $(wildcard $(images_dir)/**/*.pdf) \
	  $(wildcard images/*.jpg) $(wildcard $(images_dir)/**/*.jpg) \
	  $(wildcard $(images_dir)/*.png) $(wildcard $(images_dir)/**/*.png) \
	  $(wildcard *.sty) \
	  Makefile
bib= \
	 $(wildcard $(ref_dir)/*.bib) $(wildcard $(ref_dir)/**/.bib)


all: $(targets) 

%.pdf: %.tex $(bib) $(deps) | build
	date > build/buildlog_$@.txt;
	printf "compling $@\n" >> build/buildlog_$@.txt
	# first we run pdflatex
	cd build && TEXINPUTS=..:${TEXINPUTS} pdflatex -draftmode ../$<
	# now we need to know if we need to run bibtex or bib. For this we check if
	# the aux file contains cite commands. If so we check if there is a bcf
	# file, in which case we run biber. otherwise we run bibtex.
	cd build; \
	if grep -qE "citation\{|cite\{" $(subst .pdf,.aux,$@); then \
	printf "$@: compiling biblio with " | tee -a buildlog_$@.txt; \
	if [ -f $(subst .pdf,.bcf,$@) ]; then \
	printf "biber\n" | tee -a buildlog_$@.txt; \
	biber --input-directory=.. $(subst .pdf,,$@); \
	else \
	printf "bibtex\n" | tee -a buildlog_$@.txt; \
	BIBINPUTS=..:${BIBINPUTS} BSTINPUTS=..:${BSTINPUTS} \
	bibtex $(subst .pdf,,$@); \
	fi; \
	TEXINPUTS=..:${TEXINPUTS} pdflatex -draftmode ../$<; \
	else \
	printf "$@: no biblio\n" | tee -a buildlog_$@.txt; \
	fi;
	cd build && TEXINPUTS=..:${TEXINPUTS} pdflatex ../$< 
	# the pdf should be complete at this point. ideally we use gs now to get
	# the images to reasonable sizes. if not we just move it to the main
	# directory
	if [ $(use_gs) = 1 ]; then \
	printf "Running ghostscript\n" | tee -a build/buildlog_$@.txt; \
	gs -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dPDFSETTINGS=/prepress \
	-sOutputFile=$@ build/$@ || mv build/$@ .; \
	du -sh $@ build/$@; \
	else \
	printf "No ghostscript\n" | tee -a build/buildlog_$@.txt; \
	mv build/$@ . ; \
	fi;
	@if [ $(fail_on_missing_refs) = 1 ]; then \
	printf "I'll fail on missing reference ...\n" | tee -a build/buildlog_$@.txt; \
	if (grep "There were undefined references\|citations" build/$(subst .pdf,.log,$@) \
	 || grep "biblatex Warning: The following entry could not be found" \
	 build/$(subst .pdf,.log,$@) ); then \
	printf "BUILD FAILED because of undefined references or citations in $<\n" | \
	tee -a build/buildlog_$@.txt; \
	false; \
	else \
	printf "BUILD SUCEEDED There were no undefined references or citations\n" | \
	tee -a build/buildlog_$@.txt; \
	fi; \
	else printf "Not checking for undefined references or citations\n" | \
	tee -a build/buildlog_$@.txt; \
	fi;

test:
	echo "cloning and testing in: $$TMPDIR/temp_test_dir"
	rm -rf $$TMPDIR/temp_test_dir
	curdir=$$(pwd) && \
	cd $$TMPDIR && \
	git clone "$$curdir" temp_test_dir && \
	cd temp_test_dir && \
	make use_gs=$(use_gs) fail_on_missing_refs=$(fail_on_missing_refs)
	@echo "successfully tested in: $$TMPDIR/temp_test_dir"

build:
	mkdir -p build

debug:
	@echo "--- Evironment variables ------------------"
	@echo "USE_GS: $$USE_GS"
	@echo "FAIL_ON_MISSING_REFS: $$FAIL_ON_MISSING_REFS"
	@echo "--- Switches ------------------------------"
	@echo "use_gs: $(use_gs)"
	@echo "fail_on_missing_refs: $(fail_on_missing_refs)"
	@echo "--- Targets -------------------------------"
	@echo $(targets) | tr " " "\n"
	@echo "--- Bibs ----------------------------------"
	@echo $(bib) | tr " " "\n"
	@echo "--- Deps ----------------------------------"
	@echo $(deps) | tr " " "\n"


clean: buildclean

buildclean:
	rm -rf build  

distclean: buildclean
	rm -f $(targets)

.PHONY: all clean buildclean distclean debug test


